Generating Uncontextualized and Contextualized Questions for Document-Level Event Argument Extraction

This paper presents multiple question generation strategies for document-level event argument extraction. These strategies do not require human involvement and result in uncontextualized questions as well as contextualized questions grounded on the event and document of interest. Experimental results show that combining uncontextualized and contextualized questions is beneficial, especially when event triggers and arguments appear in different sentences. Our approach does not have corpus-specific components, in particular, the question generation strategies transfer across corpora. We also present a qualitative analysis of the most common errors made by our best model.

==> figs/da_gpt3.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		Secretary of State Hillary Clinton has taken a hard line against Iran's nuclear ambitions, recently thwarting \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated between the two countries. \textcolor{teal}{\argsubg{Clinton}{violator}} has pushed for punishing sanctions, as she argued that any negotiated settlement was not enough to ensure \textcolor{teal}{\argsubg{Iran}{otherparticipant}} would not pursue nuclear weapons. Her opposition to the agreements was based on Iran's offer to swap its low-enriched uranium for nuclear isotopes, which she felt was not sufficient to prevent their potential proliferation. Iran initially sought to refine the uranium to the levels necessary for energy production, but Clinton insisted that the sanctions remain in place. As the situation between Iran and the United States continues to evolve, Clinton's hard-line stance on the Iranian nuclear issue remains.}}

==> figs/da_lc1.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		 As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, \textcolor{teal}{\argsubg{she}{violator}} led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/da_lc2.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		As Secretary of State, \textcolor{teal}{\argsubg{Hillary Clinton}{violator}} was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/da_original.tex <==
\framebox(4.2in,1in){}

==> figs/da_pegasus.tex <==
\framebox(4.4in,1.5in){\parbox{4.3in}{
		Hillary Clinton was a strong supporter of the Iranian nuclear issue as Secretary of State. She led the opposition to any negotiated settlement and pushed for punishing sanctions after Iran indicated a willingness to compromise. \textcolor{teal}{\argsubg{Clinton}{violator}} helped sink \textcolor{red}{\argsubg{agreements}{event}} that would have allowed \textcolor{teal}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. Iran only refined about 3 - 4 percent of its nuclear material in 2009, as needed for energy production. Much of that was offered to be used for medical research.}}

==> figs/da_sw1.tex <==
%\framebox(4.4in,1.5in){\parbox{4.3in}{
\textcolor{teal}{\argsubg{Clinton}{violator}} As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.%}%}

==> figs/da_sw2.tex <==
\framebox(4.4in,1.65in){\parbox{4.3in}{
		The violator of the event \textcolor{red}{agreements} is \textcolor{teal}{\argsubg{Clinton}{violator}}. As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.}}

==> figs/rams_example.tex <==
\vspace{1.5in}

==> tables/data_augmentation.tex <==
\def\w{.5in}

\begin{tabular}{l p{4.5in}}
\toprule

Original from RAMS
&
As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, \textcolor{blue}{\argsubg{Clinton}{violator}} helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.\\ \midrule

Augmented instances \\

~~~Simple Swapping \\
~~~~~~Plain
& 
\textcolor{teal}{\argsubg{Clinton}{violator}} As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.\\ \addlinespace

~~~~~~Verbose
&
The violator of the event \textcolor{red}{agreements} is \textcolor{teal}{\argsubg{Clinton}{violator}}. As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research. \\ \addlinespace \addlinespace


~~~Leveraging Coreference  \\
~~~~~~Random mention
&
 As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, \textcolor{teal}{\argsubg{she}{violator}} led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.\\ \addlinespace

~~~~~~Meaningful mention
&
As Secretary of State, \textcolor{teal}{\argsubg{Hillary Clinton}{violator}} was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, Clinton helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.\\ \bottomrule

\end{tabular}


==> tables/data_augmentation_llms.tex <==
\def\w{.5in}

\begin{tabular}{l p{4.5in}}
\toprule

Original from RAMS
&
As Secretary of State, Hillary Clinton was a hawk on the Iranian nuclear issue. In 2009 - 2010, when Iran first indicated a willingness to compromise, she led the opposition to any negotiated settlement and pushed for punishing sanctions. To clear the route for sanctions, \textcolor{blue}{\argsubg{Clinton}{violator}} helped sink \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated with \textcolor{blue}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. In 2009, Iran was refining uranium only to the level of about 3-4 percent, as needed for energy production. Its negotiators offered to swap much of that for nuclear isotopes for medical research.\\ \midrule

Augmented instances \\


~~~Leveraging LLMs \\
~~~~~~Pegasus
&
Hillary Clinton was a strong supporter of the Iranian nuclear issue as Secretary of State. She led the opposition to any negotiated settlement and pushed for punishing sanctions after Iran indicated a willingness to compromise. \textcolor{teal}{\argsubg{Clinton}{violator}} helped sink \textcolor{red}{\argsubg{agreements}{event}} that would have allowed \textcolor{teal}{\argsubg{Iran}{otherparticipant}} to ship most of its low - enriched uranium out of the country. Iran only refined about 3 - 4 percent of its nuclear material in 2009, as needed for energy production. Much of that was offered to be used for medical research. \\ \addlinespace

~~~~~~GPT3 
&
Secretary of State Hillary Clinton has taken a hard line against Iran's nuclear ambitions, recently thwarting \textcolor{red}{\argsubg{agreements}{event}} tentatively negotiated between the two countries. \textcolor{teal}{\argsubg{Clinton}{violator}} has pushed for punishing sanctions, as she argued that any negotiated settlement was not enough to ensure \textcolor{teal}{\argsubg{Iran}{otherparticipant}} would not pursue nuclear weapons. Her opposition to the agreements was based on Iran's offer to swap its low-enriched uranium for nuclear isotopes, which she felt was not sufficient to prevent their potential proliferation. Iran initially sought to refine the uranium to the levels necessary for energy production, but Clinton insisted that the sanctions remain in place. As the situation between Iran and the United States continues to evolve, Clinton's hard-line stance on the Iranian nuclear issue remains. \\ \bottomrule

\end{tabular}


==> tables/results_transfer.tex <==
\begin{tabular}{l rr}
\toprule
 & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{Large} \\ \midrule
Template-based Questions                                   & 63.6\scriptsize{\(\pm\)1.24}\makebox[0pt][l]{$^{}$}                 & 64.7\scriptsize{\(\pm\)0.76}\makebox[0pt][l]{$^{}$}  \\
Best Strategy on RAMS                                      & 66.3\scriptsize{\(\pm\)0.24}\makebox[0pt][l]{$^{}$}                 & 67.7\scriptsize{\(\pm\)1.13}\makebox[0pt][l]{$^{}$}  \\

\midrule
Previous Work (Top 2) \\
~~APE~\citeyearpar{zhang-etal-2023-overlap}                                   & 66.0\scriptsize{\(\pm\)n/a}\makebox[0pt][l]{$^{}$}                 & 68.7\scriptsize{\(\pm\)n/a}\makebox[0pt][l]{$^{}$}  \\
~~SPEAE~\citeyearpar{nguyen-etal-2023-contextualized}                         & 66.2\scriptsize{\(\pm\)n/a}\makebox[0pt][l]{$^{}$}                 & 66.1\scriptsize{\(\pm\)n/a}\makebox[0pt][l]{$^{}$}  \\

 \bottomrule
\end{tabular}

==> tex/a_data_augmentation.tex <==
\section{Data Augmentation Examples}
\label{a:data_augmentation}
In this section, we demonstrate three data augmentation approaches. The goal of these data augmentation approaches was to transform intra-sentential arguments into inter-sentential arguments while generating new training instances. For demonstration purposes, we select a data sample from RAMS, featuring the event triggering word \emph{agreement} and two event arguments: \emph{Clinton}~(violator) and \emph{Iran}~(otherparticipant).

\subsection{Simple Swapping}
The simple swapping technique involves moving an intra-sentential argument to different positions (at the beginning or end position of each sentence), transforming it into an inter-sentential argument. The given example in Table \ref{t:augmentation_examples_1} has 4 sentences, so that leaves 5 different places to move the argument.
We consider the end position of the $i$th sentence and the beginning position of the $(i+1)$th sentence as the same position). Then, one position is chosen randomly from these 5 positions to replace the corresponding gold annotation. The \textit{verbose} version of the simple swapping approach follows the same procedure for determining the new position of the argument. However, in the verbose version, we replace the argument with a simple sentence such as \emph{``The violator of the event agreement is Clinton.''} It is worth noting that both versions generate grammatically incorrect sentences, but we focused on generating argument spans that are inter-sentential. 


\subsection{Leveraging Coreference Resolution}
In the coreference-based data augmentation, the first step involves identifying the coreference chains related to the given argument. In Table \ref{t:augmentation_examples_1}, the sample exhibits two coreference chains corresponding to the arguments. These chains are extracted using the spaCy library.\footnote{\href{https://spacy.io/}{spaCy}} For the argument \emph{Clinton}, the coreference chain appears as \emph{Hillary Clinton: [Hillary Clinton (sent 1), she (sent 2), Clinton (sent 3)]}. Similarly, for the argument \emph{Iran}, the coreference chain is \emph{[Iran (sent 2), Iran (sent 3), its (sent 3), the country (sent 3), Iran (sent 4)].} To generate augmented data using these coreference chains, we randomly select a mention from the coreference chain to replace the corresponding gold annotation. Alternatively, for the \textit{meaningful} mention, we prioritize the selection of the argument with the highest number of tokens, such as choosing \emph{Hillary Clinton} instead of \emph{Clinton.} It was observed that arguments associated with personal named entities (PER) got exposed to more informative spans by selecting meaningful mentions. At the same time, entities such as geopolitical entities (GPE) struggled to acquire informative span from meaningful references. In our case, replacing \emph{Iran} with \emph{the country} leads to the loss of argument information, which can impose limitations in certain contexts.  


\subsection{Leveraging LLMs for Paraphrasing}
To leverage Large Language Models (LLMs) for paraphrasing the RAMS samples, we employed both sentence-level and document-level paraphrasing techniques. Upon examining the examples from Table \ref{t:augmentation_examples_2}, we observed that sentence-level paraphrasing did not facilitate moving the intra-sentential arguments to inter-sentential arguments. This is because we could only provide one sentence as an input to the paraphraser model. However, using the GPT3 model with the prompt shown in Section \ref{ss:data_augmentation} generated samples with more inter-sentential arguments. In Table \ref{t:augmentation_examples_2},  both intra-sentential arguments (\emph{Clinton and Iran}) from the original sample successfully shifted to inter-sentential arguments. This transition of arguments across sentence boundaries demonstrates the potential of LLMs for enhancing the diversity of training data in natural language processing tasks.

\begin{table*}[h]
\small
\centering
\input{tables/data_augmentation}
\caption{Original instance from RAMS and additional instances obtained with our data augmentation strategies (\emph{Simple Swapping} and \emph{Leveraging Coreference}).
See descriptions of the strategies in Section \ref{ss:data_augmentation}).
While \emph{Simple Swapping} results in ungrammatical text as it shuffles intra-sentential arguments, it is the strategy that yields the best results (Table \ref{t:results}).
Leveraging coreference introduces errors.}
\label{t:augmentation_examples_1}
\end{table*}

\begin{table*}[h]
\small
\centering
\input{tables/data_augmentation_llms}
\caption{Original instance from RAMS and additional instances obtained with our data augmentation strategies (\emph{Leveraging LLMs}).
See descriptions of the strategies in Section \ref{ss:data_augmentation}).}
\label{t:augmentation_examples_2}
\end{table*}

